Perceptual error optimization for Monte Carlo animation rendering

Independently estimating pixel values in Monte Carlo rendering results in a perceptually sub-optimal white-noise distribution of error in image space. Recent works have shown that perceptual fidelity can be improved significantly by distributing pixel error as blue noise instead. Most such works have focused on static images, ignoring the temporal perceptual effects of animation display. We extend prior formulations to simultaneously consider the spatial and temporal domains, and perform an analysis to motivate a perceptually better spatio-temporal error distribution. We then propose a practical error optimization algorithm for spatio-temporal rendering and demonstrate its effectiveness in various configurations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> notused.tex <==
% \newcommand{\convolution}{\circledast}
\newcommand{\convolution}{*}
\newcommand{\Kernel}{g}
\newcommand{\KernelSpace}{\Kernel_\text{s}}
\newcommand{\KernelTime}{\Kernel_\text{t}}
\newcommand{\KernelTAA}{\Kernel_\text{a}}
\newcommand{\KernelTimeCombined}{\Kernel_\text{ta}}
\newcommand{\KernelTimeSustained}{\Kernel_{\text{t}_\text{sustained}}}
\newcommand{\KernelTimeTransient}{\Kernel_{\text{t}_\text{transient}}}

\newcommand{\FrameCount}{N}
\newcommand{\Reference}{I}
\newcommand{\ReferenceSequence}{\mathbf{\Reference}}
\newcommand{\Image}{Q}
\newcommand{\ImageSequence}{\mathbf{\Image}}
\newcommand{\Estimate}{R}
\newcommand{\EstimateSequence}{\mathbf{\Estimate}}
\newcommand{\Samples}{S}
\newcommand{\SamplesSequence}{\mathbf{\Samples}}
\newcommand{\ErrorImage}{\epsilon}
\newcommand{\ErrorImageSequence}{\mathbf{\ErrorImage}}
\newcommand{\Error}{E}
\newcommand{\ErrorSequence}{\mathbf{\Error}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{pseudocode}[t]
    \caption{
        Pseudo-code for our spatio-temporal sample-mask optimization algorithm.
    }
    \label{alg:AwesomeSauce}
    \vspace{2mm}
    \hrule height 0.7pt
    \vspace{0.5mm}
    \begin{algorithmic}[1]
        \Function{SpatioTemporalOptimize}{some params...}
            \State $\SamplesSequence = $ \todo{initialize somehow} \AlgCommentLeft{Initialize solution permutation}
            \For{$T$ iterations}
                \For{pixel $i = 1..N$} \AlgCommentLeft{E.g., random or serpentine order}
                    \State $a' = a$ \AlgCommentDown{Find best pixel in neighborhood to swap with}
                    \For{pixel $i$ in $(2)^2$ neighborhood around $i$}
                        \If{$true$} \AlgCommentLeft{huh}
                            \State $a = c$ \AlgCommentLeft{Accept swap as current best} \vspace{-0.85mm}
                        \EndIf
                    \EndFor
                    \State $a = b'$
                \EndFor
            \EndFor
            \State \Return $\SamplesSequence$
        \EndFunction{}
    \end{algorithmic}
    \vspace{0.5mm}
    \hrule height 0.7pt
\end{pseudocode}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
